A Scalable Configuration-Interaction Impurity Solver via Active Learning

Finite-Hamiltonian impurity solvers provide direct real-frequency spectra and a natural route to enlarged impurity Hamiltonians, but their applicability is limited by the rapid Hilbert-space growth with the number of bath or other added one-particle orbitals. We introduce an active-learning extension of adaptive-truncation configuration interaction (AL-ATCI) that identifies the determinant manifold relevant to the correlated state. The approximation is systematically controlled by the query size N_query, which also provides an internal convergence parameter when no external benchmark is available. Over the benchmark range studied here, the computational cost grows only weakly with bath size, because enlarging the bath mainly expands the combinatorial determinant space rather than the physically relevant manifold. In dynamical mean-field-theory benchmarks for the one-dimensional Hubbard model, AL-ATCI reproduces exact-diagonalization accuracy and extends cellular calculations to clusters as large as N_c = 10. For a three-orbital rotationally invariant Sr2RuO4 impurity problem, we demonstrate systematic convergence of dynamical quantities and a highly compressed configuration space as N_b is increased from 9 to 18. These results substantially alleviate the bath-discretization bottleneck of exact-diagonalization- and configuration-interaction-based impurity solvers and make large-bath and enlarged-orbital calculations more practical.

==> figures/supplement_body.tex <==
\section{Implementation Details of AL-ATCI}
Each configuration is represented as a binary vector encoding the spin-orbital occupations of all single-particle states.
The training labels are assigned based on the magnitude of the wavefunction coefficient: configurations whose absolute coefficient exceeds a threshold are labeled as important, and all remaining configurations as unimportant; in the present work, we use a threshold of $10^{-6}$.
Because important configurations constitute a small fraction of the total candidate space, the training set is severely class-imbalanced; we address this by assigning class weights inversely proportional to the number of samples in each class.

When the top $N_{\text{query}}$ configurations are selected, their time-reversal partners are appended to preserve time-reversal symmetry.
As a result, the total number of Slater determinants $N_{\text{SD}}^{\text{G.S.}}$ in the ground-state wavefunction can exceed $N_{\text{query}}$; the ratio $N_{\text{SD}}^{\text{G.S.}}/N_{\text{query}}$ does not substantially exceed unity in practice, as shown in Table~\ref{nSD}.

The training dataset accumulates across AL-ATCI iterations within a single DMFT cycle and is reset at the beginning of each new DMFT cycle.
This reset is necessary because updated bath parameters alter the hybridization structure, rendering the configuration importance data from the previous cycle unrepresentative of the new impurity problem.

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/Figure_S1.pdf}
    \caption{Flowchart of AL-ATCI, highlighting the active learning enhancements: classifier training, configuration importance evaluation, and selective querying of top-ranked configurations.}
    \label{fig:flowchart}
\end{figure}

\clearpage

\begin{figure}[tbph]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S2.pdf}
\caption{Convergence of the impurity self-energy with increasing $N_{\text{query}}$ at $U/t = 2$.
Top row: $\text{Im}\,\Sigma(\omega)$ on the real-frequency axis.
Bottom row: $\text{Im}\,\Sigma(i\omega_n)$ on the Matsubara-frequency axis, shown for 512 Matsubara frequencies at $\beta t = 128$.
AL-ATCI results for $N_{\text{query}} = 256, 1024, 4096, 16384$, and $65536$ (blue lines) are compared against the ED benchmark (red dashed lines).
Parameters: $N_c = 4$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:selfenergy_u2.0}
\end{figure}

\section{Self-Energy Convergence with Query Size $N_{\text{query}}$}
In the main text, Fig.~1 demonstrates that various physical quantities computed with AL-ATCI converge to exact diagonalization (ED) results as the number of active learning queries $N_{\text{query}}$ increases.
Here we extend this analysis to the impurity self-energy, shown on both the real- and Matsubara-frequency axes as $\Sigma(\omega+i\epsilon)$ and $\Sigma(i\omega_n)$.
Figure~\ref{fig:selfenergy_u2.0} shows the imaginary part of the self-energy on both the real and Matsubara frequency axes for $N_c = 4$, $N_b = 8$, at $U/t = 2$, with columns corresponding to $N_{\text{query}} = 256, 1024, 4096, 16384$, and $65536$.
Figure~\ref{fig:selfenergy_u8.0} shows the same quantities at $U/t = 8$, with columns corresponding to $N_{\text{query}} = 64, 256, 1024, 4096$, and $16384$.
In both cases, the AL-ATCI results (blue lines) systematically converge toward the ED benchmark (red dashed lines) as $N_{\text{query}}$ increases, and the Matsubara-frequency self-energy converges more rapidly than its real-frequency counterpart.

At $U/t = 2$, the result at $N_{\text{query}} = 256$ exhibits a violation of causality, which is restored from $N_{\text{query}} = 1024$ onward.
The AL-ATCI and ED self-energies become visually indistinguishable at $N_{\text{query}} = 65536$, requiring a larger $N_{\text{query}}$ than the $U/t = 8$ case.

At $U/t = 8$, the ground state CI expansion is sparse, with a small number of configurations carrying most of the weight, making it particularly amenable to the adaptive truncation strategy of AL-ATCI.
The result at $N_{\text{query}} = 64$ violates causality, and although causality is restored at $N_{\text{query}} = 256$, quantitative discrepancies with the ED benchmark persist at intermediate frequencies.
These discrepancies are systematically reduced with increasing $N_{\text{query}}$, and the AL-ATCI and ED self-energies become visually indistinguishable at $N_{\text{query}} = 4096$.
Notably, this convergence is achieved at a smaller $N_{\text{query}}$ than the $U/t = 2$ case, suggesting that AL-ATCI is particularly efficient for insulating systems where the ground state is dominated by a smaller number of important configurations.

These results confirm that AL-ATCI provides systematically improvable approximations to the self-energy across both the metallic and insulating regimes.
The convergence rate reflects the underlying correlation strength and ground-state structure, with insulating systems requiring fewer configurations to reach convergence than their metallic counterparts.
The corresponding convergence of $\text{Im}\,G_{\text{imp}}$ on both frequency axes is shown in Figs.~\ref{fig:gimp_u2.0} and~\ref{fig:gimp_u8.0}, exhibiting the same systematic behavior.

Figure~\ref{fig:convergence_Nq} further illustrates this convergence for varying broadening $\epsilon$.
The top row shows $\mathcal{E}_{\Sigma}$ as a function of $N_{\text{query}}$ for five broadening values $\epsilon = 0.02$--$0.1t$: in all cases the deviation decreases monotonically, and the onset of causality (red vertical line) occurs at a consistent $N_{\text{query}}$, confirming that the convergence behavior is robust across broadening values.
The bottom row shows $\log_{10}(\mathrm{DOS})$ at the lower Hubbard band, where the spectral features converge systematically toward the ED reference with increasing $N_{\text{query}}$.
Note that the two smallest broadening values ($\epsilon = 0.02t$ and $0.04t$) are sufficiently small that even the ED reference can exhibit causality violations; for the remaining values $\epsilon = 0.06$--$0.1t$, the $N_{\text{query}}$ at which causality is first restored (red vertical line) is consistent across broadening values, confirming that the convergence behavior of AL-ATCI is largely insensitive to the choice of $\epsilon$.


\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S3.pdf}
\caption{Convergence of the impurity self-energy with increasing $N_{\text{query}}$ at $U/t = 8$.
Top row: $\text{Im}\,\Sigma(\omega)$ on the real-frequency axis.
Bottom row: $\text{Im}\,\Sigma(i\omega_n)$ on the Matsubara-frequency axis, shown for 512 Matsubara frequencies at $\beta t = 128$.
AL-ATCI results for $N_{\text{query}} = 64, 256, 1024, 4096$, and $16384$ (blue lines) are compared against the ED benchmark (red dashed lines).
At $N_{\text{query}} = 64$, the real-frequency self-energy exhibits a causality violation, which is resolved from $N_{\text{query}} = 256$ onward.
Parameters: $N_c = 4$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:selfenergy_u8.0}
\end{figure}

\begin{figure}[tbph]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S2_added.pdf}
\caption{Convergence of the impurity Green's function with increasing $N_{\text{query}}$ at $U/t = 2$.
Top row: $\text{Im}\,G_{\text{imp}}(\omega)$ on the real-frequency axis.
Bottom row: $\text{Im}\,G_{\text{imp}}(i\omega_n)$ on the Matsubara-frequency axis, shown for 512 Matsubara frequencies at $\beta t = 128$.
AL-ATCI results for $N_{\text{query}} = 256, 1024, 4096, 16384$, and $65536$ (blue lines) are compared against the ED benchmark (red dashed lines).
Parameters: $N_c = 4$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:gimp_u2.0}
\end{figure}

\begin{figure}[tbph]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S3_added.pdf}
\caption{Convergence of the impurity Green's function with increasing $N_{\text{query}}$ at $U/t = 8$.
Top row: $\text{Im}\,G_{\text{imp}}(\omega)$ on the real-frequency axis.
Bottom row: $\text{Im}\,G_{\text{imp}}(i\omega_n)$ on the Matsubara-frequency axis, shown for 512 Matsubara frequencies at $\beta t = 128$.
AL-ATCI results for $N_{\text{query}} = 64, 256, 1024, 4096$, and $16384$ (blue lines) are compared against the ED benchmark (red dashed lines).
Parameters: $N_c = 4$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:gimp_u8.0}
\end{figure}

\begin{table}[htbp]
\centering
\begin{tabular}{rr|rr}
\hline
\multicolumn{2}{c|}{$U/t=2$} & \multicolumn{2}{c}{$U/t=8$} \\
\hline
$N_{\text{query}}$ & $N_{\text{SD}}^{\text{G.S.}}$ & $N_{\text{query}}$ & $N_{\text{SD}}^{\text{G.S.}}$ \\
\hline
$256$      & $268$      & $64$       & $84$ \\
$1\,024$   & $1\,242$   & $256$      & $284$ \\
$4\,096$   & $4\,350$   & $1\,024$   & $1\,186$ \\
$16\,384$  & $18\,574$  & $4\,096$   & $4\,469$ \\
$65\,536$  & $74\,518$  & $16\,384$  & $18\,866$ \\
\hline
\end{tabular}
\caption{Number of Slater determinants contributing to the ground state.
$N_{\text{query}}$ denotes the number of queried configurations in the selected-CI procedure, while $N_{\text{SD}}^{\text{G.S.}}$ is the number of Slater determinants with nonzero weight in the resulting ground-state wavefunction.
Because time-reversal symmetry is enforced, each queried configuration generates its time-reversed partner, so that $N_{\text{SD}}^{\text{G.S.}}$ can be larger than $N_{\text{query}}$.
Results are shown for $U/t=2$ and $U/t=8$.}
\label{nSD}
\end{table}

\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S4.pdf}
\caption{Convergence of AL-ATCI with increasing $N_{\text{query}}$ at $U/t = 8$ for different broadening values.
Each column corresponds to a distinct broadening $\epsilon = 0.02, 0.04, 0.06, 0.08, 0.1$ (in units of $t$) from left to right.
Top row: mean squared Frobenius norm of the real-frequency self-energy deviation
$\mathcal{E}_{\Sigma}=\frac{1}{N_c^2 N_\omega}\sum_m \|\Delta\boldsymbol{\Sigma}(\omega_m + i\epsilon)\|_F^2$ as a function of $N_{\text{query}}$.
The red vertical line marks the value of $N_{\text{query}}$ at which the causality condition $\mathrm{Im}\,\Sigma(\omega) \leq 0$ is first satisfied.
Bottom row: $\log_{10}(\mathrm{DOS})$ for ED (grey) and AL-ATCI with $N_{\text{query}} = 64$ (blue), $256$ (orange), $1024$ (green), $4096$ (red), and $16384$ (purple).
Parameters: $N_c = 4$, $N_b = 8$, half-filling.}
\label{fig:convergence_Nq}
\end{figure}

\clearpage

\section{Details of Scalability Measurement}
Each data point in Fig.~2 of the main text corresponds to the minimum number of configurations $N_{\text{SD}}^{\text{G.S.}}$ for which the resulting self-energy satisfies the causality condition $\mathrm{Im}\,\Sigma(\omega) \leq 0$ for all frequencies, together with the corresponding wall-clock time.
All timing measurements were performed on a single node equipped with two Intel Xeon Platinum 8360Y processors (36 cores each, 72 cores in total, 2.40\,GHz base clock, 48\,KiB L1d and 32\,KiB L1i per core, 1.25\,MiB L2 per core, 54\,MiB L3 per socket), using OpenMP parallelization across all available cores.
Timing measurements are restricted to the first five CI iterations to ensure a consistent comparison across system sizes.
This restriction is necessary because the selected configuration space can evolve differently in later iterations as the natural-orbital basis and the training dataset both evolve, making a direct comparison between AL-ATCI and ATCI ambiguous beyond the early iterations.
Figures~\ref{fig:timing_nb} and~\ref{fig:timing_nc} show the breakdown of wall-clock time into ground-state diagonalization $t_{\text{G.S.}}$, impurity Green's function evaluation $t_{G_{\text{imp}}}$, and bare Green's function evaluation $t_{G_0}$, as a function of $N_b$ and $N_c$, respectively, confirming that diagonalization dominates the total cost in both ATCI and AL-ATCI.
The remaining contributions---particle-hole substitution enumeration, Hamiltonian construction, and the machine-learning train/predict overhead---are too small to be visible on the scale of the figures and are therefore not shown separately.

\begin{figure}[htbp]
\centering
\includegraphics[width=0.6\textwidth]{figures/Figure_S5.pdf}
\caption{Cumulative wall-clock time as a function of bath size $N_b$ for ATCI (left) and AL-ATCI (right).
Three timing components are shown: ground-state diagonalization $t_{\text{G.S.}}$, impurity Green's function evaluation $t_{G_{\text{imp}}}$, and bath Green's function evaluation $t_{G_0}$.
The shaded region highlights the gap between $t_{\text{G.S.}}$ and the Green's function timings, indicating the relative cost of diagonalization.
Parameters: $N_c = 8$, half-filling, $U/t = 8$, zero temperature.}
\label{fig:timing_nb}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.6\textwidth]{figures/Figure_S6.pdf}
\caption{Cumulative wall-clock time as a function of cluster size $N_c$ for ATCI (left) and AL-ATCI (right).
Three timing components are shown: ground-state diagonalization $t_{\text{G.S.}}$, impurity Green's function evaluation $t_{G_{\text{imp}}}$, and bath Green's function evaluation $t_{G_0}$.
The shaded region highlights the gap between $t_{\text{G.S.}}$ and the Green's function timings, indicating the relative cost of diagonalization.
Parameters: $N_b = 8$, half-filling, $U/t = 8$, zero temperature.}
\label{fig:timing_nc}
\end{figure}

\clearpage

\section{Momentum-Resolved Spectral Function Convergence}
Here we examine how the momentum-resolved spectral function $A(k,\omega)$ evolves with increasing cluster size, complementing Fig.~3 of the main text.
To demonstrate the systematic convergence of AL-ATCI with increasing cluster size, we compute momentum-resolved spectral functions $A(k, \omega)$ for various cluster sizes at representative momentum points in the Brillouin zone.

Figure~\ref{fig:spectral_small} shows the spectral functions at three momentum points ($k = 0, \pi/2, \pi$) for cluster sizes $N_c = 1, 2, 4$.
As $N_c$ increases, the spectral features evolve systematically, with peak positions, heights, and spectral weights showing clear convergence with cluster size.
In particular, the spurious midgap spectral weight present at $N_c = 1$ vanishes for larger $N_c$, consistent with the Mott-insulating phase at $U/t = 8$.
The particle-hole symmetry $A(k,\omega) = A(\pi-k,-\omega)$ is clearly satisfied: the spectra at $k=0$ and $k=\pi$ are mirror images of each other under $\omega \rightarrow -\omega$, while the spectrum at $k=\pi/2$ is symmetric about $\omega=0$.
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S7.pdf}
\caption{Momentum-resolved spectral functions $A(k, \omega)$ for cluster sizes $N_c = 1$ (blue), $N_c = 2$ (orange), and $N_c = 4$ (green) at three representative momentum points.
From left to right: $k = 0$, $\pi/2$, $\pi$.
Parameters: $U/t = 8$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:spectral_small}
\end{figure}

Figure~\ref{fig:spectral_large} extends this analysis to larger cluster sizes $N_c = 6, 8, 10$, which are inaccessible to conventional ED due to the exponential growth of the Hilbert space.
The spectral functions at $N_c=8$ and $N_c=10$ differ only weakly from those at $N_c=6$, indicating that the spectra are already close to convergence by $N_c=6$.
The particle-hole symmetry $A(k,\omega) = A(\pi-k,-\omega)$ is again clearly preserved across all cluster sizes.
\begin{figure}[htbp]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S8.pdf}
\caption{Momentum-resolved spectral functions $A(k, \omega)$ for cluster sizes $N_c = 6$ (blue), $N_c = 8$ (orange), and $N_c = 10$ (green) at three representative momentum points.
From left to right: $k = 0$, $\pi/2$, $\pi$.
Parameters: $U/t = 8$, $N_b = 8$, half-filling, broadening $\epsilon = 0.1t$.}
\label{fig:spectral_large}
\end{figure}

These results confirm that AL-ATCI achieves systematic convergence of the momentum-resolved spectral function with increasing $N_c$, correctly reproducing the Mott gap and the particle-hole symmetry of the half-filled Hubbard model at $U/t = 8$.
The ability to reach cluster sizes well beyond the reach of conventional ED demonstrates the practical advantage of the active learning approach in accessing the large-$N_c$ regime.

\clearpage

\section{Slater-Kanamori Hamiltonian and Spectral Function of $\text{Sr}_2\text{RuO}_4$}
In the Sr$_2$RuO$_4$ calculations presented in the main text, the local interaction is described by the rotationally invariant Slater-Kanamori Hamiltonian for the $t_{2g}$ manifold,
\begin{align}
H_{\text{int}} &= U \sum_{m} n_{m\uparrow} n_{m\downarrow}
+ U' \sum_{m < m'} \sum_{\sigma \sigma'} n_{m\sigma} n_{m'\sigma'} \notag \\
&\quad - J \sum_{m < m'} \sum_{\sigma \sigma'} c^{\dagger}_{m\sigma} c_{m\sigma'} c^{\dagger}_{m'\sigma'} c_{m'\sigma} \notag \\
&\quad + J \sum_{m < m'} \left( c^{\dagger}_{m\uparrow} c^{\dagger}_{m\downarrow} c_{m'\downarrow} c_{m'\uparrow} + \text{H.c.} \right),
\end{align}
where $m, m' \in \{d_{xy}, d_{xz}, d_{yz}\}$ label the $t_{2g}$ orbitals, $\sigma$ denotes spin, and $n_{m\sigma} = c^{\dagger}_{m\sigma} c_{m\sigma}$.
The parameters $U$, $U' = U - 2J$, and $J$ denote the intraorbital Coulomb repulsion, interorbital Coulomb repulsion, and Hund's coupling, respectively.
The relation $U' = U - 2J$ ensures rotational invariance in orbital space.
In the main text, we use $U = 2.5$\,eV and $J = 0.4$\,eV.
Figure~\ref{fig:SRO_SM} shows the zero-temperature spectral function for $N_b = 9, 12, 15, 18$.
Both $xy$ and $xz/yz$ components converge systematically with increasing bath size, displaying well-defined quasiparticle bands near the Fermi level and incoherent weight at higher energies, consistent with the correlated metallic state of Sr$_2$RuO$_4$.
This confirms that the weak bath-size dependence observed in the single-band case extends to the three-orbital rotationally invariant problem.
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/Figure_S9.png}
\caption{Spectral function of Sr$_2$RuO$_4$ from zero-temperature single-site DMFT with AL-ATCI, for $U = 2.5$\,eV and $J = 0.4$\,eV.
As $N_b$ increases from 9 to 18, the spectral function converges systematically, confirming that AL-ATCI's weak bath-size dependence extends to a three-orbital problem with the full rotationally invariant interaction.}
\label{fig:SRO_SM}
\end{figure}

